Laser Cooling of Transition Metal Atoms

We propose the application of laser cooling to a number of transition-metal atoms, allowing numerous bosonic and fermionic atomic gases to be cooled to ultra-low temperatures. The non-zero electron orbital angular momentum of these atoms implies that strongly atom-state-dependent light-atom interactions occur even for light that is far-detuned from atomic transitions. At the same time, many transition-metal atoms have small magnetic dipole moments in their low-energy states, reducing the rate of dipolar-relaxation collisions. Altogether, these features provide compelling opportunities for future ultracold-atom research. Focusing on the case of atomic titanium, we identify the metastable $a ^5F_5$ state as supporting a $J \rightarrow J+1$ optical transition with properties similar to the D2 transition of alkali atoms, and suited for laser cooling. The high total angular momentum and electron spin of this state suppresses leakage out of the the nearly closed optical transition to a branching ratio estimated below $\sim 10^{-5}$. Following the pattern exemplified by titanium, we identify optical transitions that are suited for laser cooling of elements in the scandium group (Sc, Y, La), the titanium group (Ti, Zr), the vanadium group (V, Nb), the manganese group (Mn, Tc), and the iron group (Fe, Ru).

==> table_complete.tex <==
\begin{table*}[]
    \centering
    \begin{ruledtabular}
    \begin{tabular}{cccccccccccc}
        \textbf{Atom}&\multicolumn{2}{c}{\textbf{Ground state}}& \multicolumn{4}{c}{\textbf{Metastable state}}&\multicolumn{3}{c}{\textbf{Excited state}}&&\\
        &config.&term&config.&term&energy& decay rate&config.&term&energy&Cooling&Linewidth\\
        &&&&&(\si{\per\centi\meter})&(\si{\milli\hertz})&&&(\si{\per\centi\meter})&trans. (\si{\nano\meter})&($\si{\mega\hertz}/2\pi$)\\\hline\\
        Sc\cite{sugar_atomic_1985,ben_ahmed_extension_1977,lawler_absolute_1989}&$3d4s^2$&$a^2D_{3/2}$&$3d^2(^3F)4s$&$a^4F_{9/2}$&11677.3121&\textbf{---}&$3d^2(^3F)4p$&$z^4G_{11/2}^{^\circ}$&45761.10(.05)&567.3402(15)&8.6 \\
        Y\cite{b._a._palmer_first_1977,meggers_tables_1975,hannaford_oscillator_1982}&$4d5s^2$&$a^2D_{3/2}$&$4d^2(^3F)5s$&$a^4F_{9/2}$&11532.096&\textbf{---}&$4d^2(^3F)5p$ & $z^4G_{11/2}^{^\circ}$&29820.374(13)&546.7986(4)&10.\\
        La\cite{meggers_tables_1975,martin_atomic_1978,hartog_radiative_2015}&$5d6s^2$&$^2D_{3/2}$&$5d^2(^3F)6s$&$^4F_{9/2}$&4121.572&\textbf{---} &$5d^2(^3F)6p$&$^4G_{11/2}^{^\circ}$&20117.38&625.166&5.86\\
        &&&&&&&$4f5d(^3G^{^\circ})6s$&$^4G_{11/2}^{^\circ}$&24841.42&406.148&8.9\\
        Ac\cite{moore_atomic_1971} & $6d7s^2$ & $a^2D_{3/2}$ & $6d^2(^3F)7s$ & $a^4F_{9/2}$ & 12078.07 & \textbf{---} & $6d^2(^3F)7p$ & $z^4G_{11/2}^{^\circ}$ &33429.76& 468.34\footnotemark[3] & \textbf{---} \\ \\
        Ti\cite{saloman_energy_2012,forsberg_spectrum_1991,blackwell_precision_1982,borrero_accurate_2003} & $3d^24s^2$ & $a^3F_4$ & $3d^3(^4F)4s$ & $a^5F_5$ & 6842.962 & \textbf{---} & $3d^3(^4F)4p$ & $y^5G_6^{^\circ}$ & 26910.709(5)& 498.3121(3) & 10.5 \\
        & & & & & & & $3d^24s4p$ \footnotemark[1] & $z^5G_6^{^\circ}$ & 16458.671(4)& 1039.9660(13) & 0.0113\\
        Zr\cite{meggers_tables_1975,moore_atomic_1971-1} & $4d^25s^2$ & $a^3F_4$ & $4d^3(^4F)5s$ & $a^5F_5$ & 5888.93 & \textbf{---} & $4d^3(^4F)5p$ & $y^5G_6^{^\circ}$ & 16978.29& 468.780\footnotemark[2] & \textbf{---}\\
        & & & & & & & $4d^25s5p$\footnotemark[1] & $z^5G_6^{^\circ}$ & 27214.89& 901.77\footnotemark[2] & \textbf{---}\\ \\
        %Hf & $a^3F_4$ & $a^5F_5$ & 17901 &  &  &  \\ \\
        V\cite{thorne_spectrum_2011,saloman_critically_2017,childs_hyperfine_1967,meggers_term_1936,r._l._kurucz_http://kurucz.harvard.edu/atoms/2300/_2011,holmes_experimentally_2016} & $3d^34s^2$ & $a^4F_{3/2}$ & $3d^4(^5D)4s$ & $a^6D_{9/2}$ & 2424.809(2) & 0.017 & $3d^4(^5D)4p$ & $y^6F_{11/2}^{^\circ}$ & 25253.457(2)& 438.04603(18) & 18.3 \\
        & & & & & & & $3d^34s4p$\footnotemark[1]& $z^6F_{11/2}^{^\circ}$ & 18680.070(3) & 615.1955(2) & \textbf{---} \\
        & & & $3d^4(^3H)4s$ & $a^4H_{13/2}$ & 15062.959 & \textbf{---} & $3d^4(^3H)4p$ & $z^4I_{15/2}^{^\circ}$ & 37518.445(4)&445.32548(12)&13.\\
        Nb\cite{meggers_tables_1975,moore_atomic_1971-1,kroger_new_2004} & $4d^4(^5D)5s$ & $a^6D_{1/2}$ & \textbf{---} & $a^6D_{9/2}$ & 1050.26 & \textbf{---} & $4d^4(^3H)5p$ & $y^6F_{11/2}^{^\circ}$ & 25680.36 & 405.894\footnotemark[2] & \textbf{---} \\
        & & & & & & & $4d^35s(^5F)5p$ & $z^6F_{11/2}^{^\circ}$ & 20939.92(2) & 502.6335(5)\footnotemark[2] & \textbf{---} \\
        & & & $4d^4(^3H)5s$ & $a^4H_{13/2}$ & 11524.65 & \textbf{---} & $4d^4(^3H)5p$ & $z^4I_{15/2}^{^\circ}$ & 33116.36& 463.1407& \textbf{---}\\ \\
        Mn\cite{sugar_atomic_1985,meggers_tables_1975,nussbaumer_forbidden_1972,booth_measurement_1984} & $3d^54s^2$ & $a^6S_{5/2}$ & \textbf{---} & \textbf{---} & 0 & 0 & $3d^5(^6S)4s4p(^3P^{^\circ})$ & $z^6P_{7/2}^{^\circ}$ & 24802.25 & 403.076 & 2.71 \\
        &  &  &  &  &  &  &  & $z^6P_{5/2}^{^\circ}$ & 24788.05 & 403.307 & 2.63 \\
        &  &  &  &  &  &  &  & $z^6P_{5/2}^{^\circ}$ & 24779.32 & 403.449 & 2.51 \\
        & & & $3d^6(^5D)4s$ & $a^6D_{9/2}$ & 17052.29 & 290 & $3d^6(^5D)4p$ & $z^6F_{11/2}^{^\circ}$ & 43314.23 & 380.780 & 9.4 \\
        & & & $3d^6(^3H)4s$ & $a^4H_{13/2}$ & 34138.88 & \textbf{---} & $3d^6(^3H)4p$ & $z^4I_{15/2}^{^\circ}$ & 58852.60 & 404.634\footnotemark[3] & \textbf{---} \\
        Tc\cite{bozman_energy_1968,palmeri_interpretation_1999,bozman_improved_1967} & $4d^55s^2$ & $a^6S_{5/2}$ & $4d^6(^5D)5s$ & $a^6D_{9/2}$ & 2572.89 & \textbf{---} & $4d^6(^5D)5p$ & $z^6F_{11/2}^{^\circ}$ & 30067.29 & 363.7106 & 25.0 \\
        & & & $4d^6(^3H)5s$ & $^4H_{13/2}$ & 16553.39 & \textbf{---} & $4d^6(^3H)5p$ & $^4I^{^\circ}_{15/2}$ & 42996.15 & 378.0680 &\textbf{---}\\ \\
        Fe\cite{brown_atomic_1995,nave_new_1994,blackwell_precision_1979} & $3d^64s^2$ & $a^5D_4$ & $3d^7(^4F)4s$ & $a^5F_5$ & 6928.268 & 2.0 & $3d^7(^4F)4p$ & $z^5G_6^{^\circ}$ & 26874.550(1)& 358.22150(4) & 16.2 \\
        Ru\cite{meggers_tables_1975,moore_atomic_1971,wickliffe_atomic_1994} & $4d^7(^4F)5s$ & $a^5F_5$ & \textbf{---} & \textbf{---} & 0 & 0 & $4d^7(^4F)5p$ & $z^5G_6^{^\circ}$ & 26816.23& 349.994 & 13.7 \\ \\
        %Os &  &  &  &  &  &  \\ \\
        %Ce\cite{meggers_tables_1975,martin_atomic_1978,lawler_atomic_2010} & $4f5d6s^2$ & $^1G_4^{^\circ}$ & $4f5d^26s$ \footnotemark[1] & $^5I_8^{^\circ}$ & 6809.128 & \textbf{---} & $4f5d^26p$  \footnotemark[1] & $^5K_9$ & & 570.081\footnotemark[2] & \textbf{---}
        %Th && $a^3F_4$ && $a^5F_5$ & 9804 && $z^3H_6^{^\circ}$ & 2138 & \textbf{---} \\
        \footnotetext{In Ti, Zr and V, the full electronic configuration of the excited state of the narrow cooling transitions are $3d^2(^3F)4s4p(^3P^{^{\circ}})$,  $4d^2(^3F)5s5p(^3P^{^{\circ}})$, and $3d^3(^4F)4s4p(^3P^{^\circ})$ respectively.}
        \footnotetext{References for these wavelengths was only given in air. A conversion to vacuum wavelengths was made using (INSERT FORMULA AND REFERENCE HERE).}
        \footnotetext{No measured transition, wavelength inferred from energy levels}
    \end{tabular}
    \end{ruledtabular}
    \caption{Laser cooling lines of transition metals. For each atom, the relevant references are grouped by the atom itself, instead of by each number that has been referenced}
    \label{tab:alltransitions}
\end{table*}

